Multiversion Concurrency with Bounded Delay and Precise Garbage Collection

In this paper we are interested in bounding the number of instructions taken to process transactions. The main result is a multiversion transactional system that supports constant delay (extra instructions beyond running in isolation) for all read-only transactions, delay equal to the number of processes for writing transactions that are not concurrent with other writers, and lock-freedom for concurrent writers. The system supports precise garbage collection in that versions are identified for collection as soon as the last transaction releases them. As far as we know these are first results that bound delays for multiple readers and even a single writer. The approach is particularly useful in situations where read-transactions dominate write transactions, or where write transactions come in as streams or batches and can be processed by a single writer (possibly in parallel). The approach is based on using functional data structures to support multiple versions, and an efficient solution to the Version Maintenance (VM) problem for acquiring, updating and releasing versions. Our solution to the VM problem is precise, safe and wait-free (PSWF). We experimentally validate our approach by applying it to balanced tree data structures for maintaining ordered maps. We test the transactional system using multiple algorithms for the VM problem, including our PSWF VM algorithm, and implementations with weaker guarantees based on epochs, hazard pointers, and read-copy-update. To evaluate the functional data structure for concurrency and multi-versioning, we implement batched updates for functional tree structures and compare the performance with state-of-the-art concurrent data structures for balanced trees. The experiments indicate our approach works well in practice over a broad set of criteria.

==> exp-old.tex <==
\renewcommand{\figurename}{Figure}
\section{Experiments}
\label{sec:exp}
We have implemented our wait-free algorithm for the \VerMain{} problem
and a framework for batching updates, and use it in conjunction with
the C++ PAM library~\cite{pam} to experimentally study the
effectiveness of our approach.  PAM supports functional tree
structures by path-copying, and implements a reference counting
garbage collector.

We first test the functional tree structure in the single-writer,
multi-reader concurrent setting with batched updates.  We do this for
two benchmarks.  The first is for the Yahoo!  Cloud Serving Benchmark
(YCSB)~\cite{ycsb}, which involves streams of updates and queries on a
dictionary.  By using a single writer with batched updates
our implementation outperforms other
state-of-the-art concurrent data structures in all the workloads we
tested.  The second benchmark is for document index searching, which
involves a stream of document insertion intermixed with document
search queries.  We compare this to a version based on a static
index~\cite{pam}.  Experiments show that queries and updates do not
significantly delay each other.   For these experiments we do not
use garbage collection.

We then more carefully analyze the overheads of our wait-free
\VerMain{} algorithm, and of the garbage collector by
experimenting with different settings and batch sizes.  The
experiments show that the overhead of GC and a single-thread update is
reasonably small (within 21\%), and there is hardly any contention
caused by more query threads or more frequent queries (within
10\%). These results are consistent with our theoretical results.  We
also study how the number of live versions is effected different query and update granularity---the number of versions is never more than the number of
threads, and generally much less.

We do not compare to general purpose software transactional memory systems
since previous results show they are not competitive to direct concurrent
implemenations~\cite{Gramoli15}.


\textbf{Setup.}  For all experiments, we use a 72-core Dell R930 with
4 x Intel(R) Xeon(R) E7-8867 v4 (18 cores, 2.4GHz and 45MB L3 cache),
and 1Tbyte memory.  Each core is 2-way hyperthreaded giving 144
hyperthreads.  Our code was compiled using g++ 5.4.1, which supports
the Cilk Plus extensions.  We compile with \texttt{-O2}. We use
\texttt{numactl -i all} in all experiments, evenly spreading the
memory pages across the processors in a round-robin fashion.

\begin{figure*}[!h]
  \begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c}
      (a)&\includegraphics[width=0.64\columnwidth]{../figures/ycsb.pdf}
      (b)&\includegraphics[width=0.64\columnwidth]{../figures/max-version} & %(b)&\includegraphics[width=0.64\columnwidth]{../figures/ave-version} &
      (c)&\includegraphics[width=0.64\columnwidth]{../figures/thread} \\
      %      \includegraphics[width=0.7\columnwidth]{figures/ave-version}\\
  \end{tabular}\vspace{-.1in}
  \caption{\small Some experimental results. (a). Throughput of six concurrent data structures on YCSB workloads A (read/update, 50/50), B (read/update, 95/5) and C (all reads). (b). the number of the maximum and average live versions during the whole lock-free version maintenance algorithm. (c). the query throughput (millions of queries per thread per second) when running with different query threads and granularity (different values of $n_q$). }\label{fig:augsumexp}
  \vspace*{-.2in}
\end{figure*}


\subsection{Evaluating the VM Algorithms in Our Framework}
\label{sec:exp:rangesum}
In this section, we study the performance of our wait-free \VerMain{}
algorithm and the garbage collector under various conditions.  We also
designed and tested a simple lock-free algorithm for version
maintenance, but in all cases, the lock-free algorithm is about
15-20\% slower than our wait-free algorithm so we do not include
results.

We use integer keys and values, and conduct parallel queries while
updating the tree. Each query asks for the sum of all values
in a key range.  We augment tree such that each query costs $O(\log
n)$.  The initial tree size is $n=10^8$. We use $P=141$ threads to
invoke concurrent transactions, among which one thread continually
commits updates, each containing $n_u$ sequential insertions, and
$140$ threads conduct queries, each containing $n_q$ range-sum
queries.  We control the granularity of batches of updates and queries
by adjusting $n_u$ and $n_q$.  We set the total running time to be 30
seconds, and test different combinations of update and query batch
granularity.
%Before each update happens, we record the number of living versions at that point. This will slightly affect the performance, but the difference seems to be small.
We count the maximum number of live versions before each update, and
also report the throughput of the updates and queries.

\begin{fullversion}
\begin{table}[!h!t]
  \centering
    \begin{tabular}{|r|r|r|r|r|r|}
    \hline
    \multicolumn{1}{|c|}{{\textbf{Query}}} & \multicolumn{5}{c|}{\textbf{Update Granularity}} \\
\cline{2-6} \multicolumn{1}{|c|}{{\textbf{Granularity}}}          & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{10}} & \multicolumn{1}{c|}{\textbf{100}} & \multicolumn{1}{c|}{\textbf{1000}} & \multicolumn{1}{c|}{\textbf{10000}} \\
    \hline
    \textbf{1} & 8     & 4     & 3     & 2     & 1 \\
    \hline
    \textbf{10} & 9     & 4     & 3     & 2     & 1 \\
    \hline
    \textbf{100} & 42    & 7     & 3     & 2     & 1 \\
    \hline
    \textbf{1000} & 113   & 54    & 9     & 2     & 1 \\
    \hline
    \textbf{10000} & 141   & 130   & 55    & 8     & 2 \\
    \hline
    \end{tabular}%
      \caption{The maximum number of live versions.}
  \label{tab:maxversion}%
\end{table}%

\begin{table}[!h!t]
  \centering
    \begin{tabular}{|r|r|r|r|r|r|}
    \hline
    \multicolumn{1}{|c|}{\textbf{Query}} & \multicolumn{5}{c|}{\textbf{Update Granularity}} \\
\cline{2-6}    \multicolumn{1}{|c|}{\textbf{Granularity}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{10}} & \multicolumn{1}{c|}{\textbf{100}} & \multicolumn{1}{c|}{\textbf{1000}} & \multicolumn{1}{c|}{\textbf{10000}} \\
    \hline
    \textbf{1} & 1.92  & 1.29  & 1.16  & 1.00  & 1.00  \\
    \hline
    \textbf{10} & 3.77  & 1.21  & 1.21  & 1.00  & 1.00  \\
    \hline
    \textbf{100} & 25.47  & 4.34  & 1.22  & 1.00  & 1.00  \\
    \hline
    \textbf{1000} & 81.71  & 34.56  & 4.93  & 1.03  & 1.00  \\
    \hline
    \textbf{10000} & 133.55  & 109.30  & 40.76  & 5.51  & 1.02  \\
    \hline
    \end{tabular}%
      \caption{Average number of live versions. }
  \label{tab:aveversion}%
\end{table}%
\end{fullversion}


\paragraph{The number of live versions.}
The number of live versions is shown in Figure \ref{fig:augsumexp}
(b).  When $n_u$ is small, which means the updates happen more often,
the number of live versions gets larger.  This is because new versions
are generated frequently, while the old versions are still used in
queries and not yet collected.  Accordingly, when $n_u$ is large,
update transactions take a long time and almost every query can access
the current version.  On the other hand, when the query transactions
are longer (larger $n_q$), the number of live versions also gets
larger.  This is because when a read transaction takes a long time, it
is more likely to be behind the current version, and to keep some very
old versions live.  In turn when the queries are fast, all of them may
catch some recent versions.

In all, the number of total versions is at most $140$, which appears
in when $n_u$ is small and $n_q$ is large. For not too slow queries
($n_q<10^4$) and not too fast updates ($n_u>10$), the maximum number
of versions is around $10$, which is $1/14$ of the total query
threads.  Because our GC is precise, all out-of-date versions are
collected immediately.

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\paragraph{The throughput of queries and updates.}
\begin{table}[!t]
\vspace{-.1in}
  \centering\small
\begin{tabular}{@{}c@{ }|@{ }c@{ }||c|c|c|c|c|c||c|c|c|c@{}}
\hline
 &  & \multicolumn{6}{c||}{\textbf{M queries /s}}           & \multicolumn{4}{c}{\textbf{M updates /s}} \\
\cline{3-12}
$\boldsymbol{n_q}$&   $\boldsymbol{n_u}$    & \textbf{U} & \textbf{GC} & \textbf{U} & \textbf{GC} & \textbf{U} & \textbf{GC} & \textbf{Q} & \textbf{GC} & \textbf{Q} & \textbf{GC} \\
\cline{3-12}
&       & \multicolumn{1}{c|}{\xmark} & \multicolumn{1}{c|}{\xmark} & \multicolumn{1}{c|}{\cmark} & \multicolumn{1}{c|}{\xmark} & \multicolumn{1}{c|}{\cmark} & \multicolumn{1}{c||}{\cmark} & \multicolumn{1}{c|}{\xmark} & \multicolumn{1}{c|}{\cmark} & \multicolumn{1}{c|}{\cmark} & \multicolumn{1}{c}{\cmark} \\
\hline
$\boldsymbol{10}$ & $\boldsymbol{10}$ & \multicolumn{2}{c|}{46.0} &  \multicolumn{2}{c|}{43.0} &\multicolumn{2}{c||}{35.4}& \multicolumn{2}{c|}{0.081} & \multicolumn{2}{c}{0.090} \\
\hline
$\boldsymbol{10}$ & \textbf{$\boldsymbol{10^4}$} & \multicolumn{2}{c|}{46.0}  & \multicolumn{2}{c|}{43.3} & \multicolumn{2}{c||}{35.2}& \multicolumn{2}{c|}{0.170} & \multicolumn{2}{c}{0.120} \\
\hline
\textbf{$\boldsymbol{10^4}$} & $\boldsymbol{10}$ & \multicolumn{2}{c|}{51.2} &  \multicolumn{2}{c|}{44.4} & \multicolumn{2}{c||}{36.0} &\multicolumn{2}{c|}{0.080} & \multicolumn{2}{c}{0.098} \\
\hline
\textbf{$\boldsymbol{10^4}$} & \textbf{$\boldsymbol{10^4}$} & \multicolumn{2}{c|}{51.2}  & \multicolumn{2}{c|}{44.5} & \multicolumn{2}{c||}{37.3}& \multicolumn{2}{c|}{0.175} & \multicolumn{2}{c}{0.150} \\
\hline
\multicolumn{12}{l}{U: update, Q: query, GC: garbage collection}
\end{tabular}%
    \caption{\small The throughput (millions of queries/updates per second) with varied settings. \cmark{} (\emph{yes}) and \xmark{} (\emph{no}) in the table denote if GC, updates and queries are enabled in the corresponding tests.}\label{tab:contention}
    \vspace{-.25in}
\end{table}%

We test four combinations of update and query granularity, as shown in
Table \ref{tab:contention}, and report the query and update throughput
(millions of queries/updates per second). We compare the throughput
numbers when queries and updates are executed together or on their
own. For the query throughput we also test the performance when there
is no GC.

\emph{The Query Throughput.} Introducing a single-thread update
transaction always lowers the throughput of queries. This is not only
because of the overhead in running update transactions, but also from
the possible GC cost---no update implies no new versions, and the
current version will never be collected. To illustrate the overhead
ratio of doing updates to GC, we show our algorithm without GC for
comparison (the 4th column in Table~\ref{tab:contention}).  For all
cases shown in Table \ref{tab:contention}, the overhead caused by
GC is around 20\% (comparing column 4 and 5 in the table).
%When $n_q$ is large, this overhead is slightly higher because it is more likely that the queries are keeping some very old versions, and are responsible for collecting them.

The overhead of update is reasonably small (less than 7\%) when $n_q$
is small, and can be more significant (around 15\%) when $n_q$ is
larger. This overhead is mainly due to the cache locality. When there
are no write transactions, all the query transactions are working on
the same tree, and the top levels of the tree are always cached.
Instead, if updates are running, because of path-copying, part of the
top levels are newly generated (e.g., the root is always new). This
also explains the phenomenon that the overhead caused by updates is
more significant when $n_q$ is larger. In this case, query
transactions take a long time. During the queries, the tree is updated with
more \tuple{}s, thus the top levels in the tree are mostly new, which
causes deterioration of cache performance. %Also, in general, when
%$n_q$ is small the throughput is lower because of the higher
%contention in modifying counters on the current version.

In all, the overhead caused by both the single-thread writer and GC is
reasonably small (both within 21\%) for queries.

\emph{The Update Throughput.} When $n_u$ is large, we see significant
drop in update throughput when queries are involved (about 30\%). The
overhead comes from both CASes in queries and the GC invoked by
queries---the writer attempts to increase the reference counters of
the tree nodes, while the GCs caused by the queries try to decrease
the counters.

Note that when $n_u$ is small, the throughput
of updates running by its own can be lower than when running with
queries. This is likely because when there is no query, the writer is
responsible for collecting the old versions (when queries are running,
the writer and the readers share the responsibility for GC). When
$n_u$ is small, committing new versions is very frequent, and the
overhead in GC cost can be significant.

In all, queries cause overhead to updates, but can also share the
responsibility for GC with writers and make writers faster.

\paragraph{Thread Contention Between Queries.}
We also use different number of query threads to test the contention
between threads. Results are shown in Figure \ref{fig:augsumexp}
(c). The contention mainly lies in the interaction of readers and
writers via the CASes, which has been shown to be bounded. We test
with $n_u=1000$, and try different number of $n_q$.  We report the
query throughput. Ideally when there is no contention, this quantity
should stay the same for different settings, but in practice more
working threads and faster query transactions should imply higher
contention.  Indeed for $n_q=1$, queries are frequent enough that we
can see significant overhead. However, as shown in Figure
\ref{fig:augsumexp} (c), when $n_q$ is not too small, even when
$n_q=5$, we hardly see the throughput dropping with more working
threads, meaning that there is little contention between
threads. Also, when $n_q$ is $5$ the performance is very close to when
$n_q$ is as large as $10^4$. These results are consistent with our
theory that the contention is bounded (constant amortized contention).
In all, for query transactions that are not too small (even for $n_q$
around 5), there is little contention (within 10\%) caused by using
more query threads. %, as well as caused by more frequent queries.
%For $n_q=1$, queries are too frequent such that the overhead is still significant.
\hide{
\paragraph{The throughput of queries.}
We also present the throughput of queries in Table \ref{tab:query} and Figure \ref{fig:augsumexp} (c). We compare the throughput with when there are only queries, based on our version or directly using PAM (no versioning).

First, we can see that when $n_q$ is small, increasing $n_q$ will result in larger throughput. This is because more queries are batched in one transaction, amortizing the overhead across each query. When $n_q$ gets larger, the ratio of overhead gets smaller, and thus the throughput stays almost the same for $n_q\ge 100$.

The granularity of updates does not seem to affect the query much. When there is no update, all queries will attempt to acquire the only version and use CAS to update the counter. In this case, the query throughput will even get smaller and when the queries are frequent ($n_q=1$ or $10$). %This because of the high contention on updating the counter.
%Since we know that no update will happen and the current version will never be collected, we can directly use the current version without updating the counter.
Hence we also show the performance of directly using PAM without versioning. It has significantly better performance with more frequent queries because of no contention caused by CAS.
When $n_q$ gets larger, our version with $n_u=0$ gets similar performance with PAM.

When $n_q$ is small, the overhead of adding update transactions running in background comes mainly from the contention in the contention in updating the counter. When $n_q$ is large, the overhead of maintaining the counters is only a smaller fraction comparing with the query time. In this case the overhead may come from the garbage collection.
This doe not seem to be much (around $20\%$). This means that in practice, our lock-free algorithm has very good performance: all the concurrent queries can continually get updated versions, and the overhead of this is reasonably small with a reasonable query rate comparing to the case with no updates.


\paragraph{The Throughput of Updates.}
We present the throughput of updates in Table \ref{tab:updatethroughput} and Figure \ref{fig:augsumexp} (b). We compare the throughput with when there are only updates, based on our version or directly using PAM (no versioning).

In general, less frequent query transactions give higher throughput due to less contention in updating the counter.
The throughput of directly using PAM is significantly larger than the others. This is mainly because in this case, there is no version maintenance or garbage collection, and thus all versions are preserved. This is also illustrated by the fact that when $n_u$ gets larger, the gap narrowed between the bars of PAM and $n_q=0$. This is because when new version are generated less frequent, the overhead in garbage collection also drops. Even so our lock-free algorithm achieve about a half throughput in update comparing with PAM, which need to preserve all history versions---it can be proportional to the total number of update transactions.

Another interesting observation is that, when $n_u$ is small, the update throughput without simultaneous query is even smaller than when there is query. This is because in this case, the garbage collection is mostly done by the writer, bringing down the update throughput.}


==> figures.tex <==
\hide{
\begin{table*}[!t]
\vspace{-.1in}
  \centering\small
\begin{tabular}{@{}c@{ }|@{ }c@{ }||c|c|c|c|c|c||c|c|c|c@{}}
\hline
 &  & \multicolumn{6}{c||}{\textbf{M queries /s}}           & \multicolumn{4}{c}{\textbf{M updates /s}} \\
\cline{3-12}
$\boldsymbol{n_q}$&   $\boldsymbol{n_u}$    & \textbf{U} & \textbf{GC} & \textbf{U} & \textbf{GC} & \textbf{U} & \textbf{GC} & \textbf{Q} & \textbf{GC} & \textbf{Q} & \textbf{GC} \\
\cline{3-12}
&       & \multicolumn{1}{c|}{\xmark} & \multicolumn{1}{c|}{\xmark} & \multicolumn{1}{c|}{\cmark} & \multicolumn{1}{c|}{\xmark} & \multicolumn{1}{c|}{\cmark} & \multicolumn{1}{c||}{\cmark} & \multicolumn{1}{c|}{\xmark} & \multicolumn{1}{c|}{\cmark} & \multicolumn{1}{c|}{\cmark} & \multicolumn{1}{c}{\cmark} \\
\hline
$\boldsymbol{10}$ & $\boldsymbol{10}$ & \multicolumn{2}{c|}{46.0} &  \multicolumn{2}{c|}{43.0} &\multicolumn{2}{c||}{35.4}& \multicolumn{2}{c|}{0.081} & \multicolumn{2}{c}{0.090} \\
\hline
$\boldsymbol{10}$ & \textbf{$\boldsymbol{10^4}$} & \multicolumn{2}{c|}{46.0}  & \multicolumn{2}{c|}{43.3} & \multicolumn{2}{c||}{35.2}& \multicolumn{2}{c|}{0.170} & \multicolumn{2}{c}{0.120} \\
\hline
\textbf{$\boldsymbol{10^4}$} & $\boldsymbol{10}$ & \multicolumn{2}{c|}{51.2} &  \multicolumn{2}{c|}{44.4} & \multicolumn{2}{c||}{36.0} &\multicolumn{2}{c|}{0.080} & \multicolumn{2}{c}{0.098} \\
\hline
\textbf{$\boldsymbol{10^4}$} & \textbf{$\boldsymbol{10^4}$} & \multicolumn{2}{c|}{51.2}  & \multicolumn{2}{c|}{44.5} & \multicolumn{2}{c||}{37.3}& \multicolumn{2}{c|}{0.175} & \multicolumn{2}{c}{0.150} \\
\hline
\multicolumn{12}{l}{U: update, Q: query, GC: garbage collection}
\end{tabular}%
    \caption{\small The throughput (millions of queries/updates per second) with varied settings. \cmark{} (\emph{yes}) and \xmark{} (\emph{no}) in the table denote if GC, updates and queries are enabled in the corresponding tests.}\label{tab:contention}
    \vspace{-.25in}
\end{table*}%
}

\begin{table*}[htbp]
  \centering
    \begin{tabular}{rr|rrrr|rrrr|rrr|rrr}
    \hline
    \multicolumn{1}{c}{\multirow{2}[4]{*}{$\boldsymbol{n_q}$}} & \multicolumn{1}{c|}{\multirow{2}[4]{*}{$\boldsymbol{n_u}$}} & \multicolumn{4}{c|}{\textbf{Query Throughput (M/s)}} & \multicolumn{4}{c|}{\textbf{Update Throughput (M/s)}} & \multicolumn{3}{c|}{\textbf{Max \# Version}} & \multicolumn{3}{c}{\textbf{Ave. \# Version}} \\
\cline{3-16}          &       & \multicolumn{1}{c}{\textbf{Base}} & \multicolumn{1}{c}{\textbf{Ours}} & \multicolumn{1}{c}{\textbf{HP}} & \multicolumn{1}{c|}{\textbf{EP}} & \multicolumn{1}{c}{\textbf{Base}} & \multicolumn{1}{c}{\textbf{Ours}} & \multicolumn{1}{c}{\textbf{HP}} & \multicolumn{1}{c|}{\textbf{EP}} & \multicolumn{1}{c}{\textbf{Ours}} & \multicolumn{1}{c}{\textbf{HP}} & \multicolumn{1}{c|}{\textbf{EP}} & \multicolumn{1}{c}{\textbf{Ours}} & \multicolumn{1}{c}{\textbf{HP}} & \multicolumn{1}{c}{\textbf{EP}} \\
    \hline
    \textbf{10} & \textbf{10} &  43.15     & 37.08 & 37.41 & \underline{37.88} &  0.119     & \underline{0.097} & 0.054 & 0.056 & \underline{4}     & 282   & 194   & \underline{1.11}  & 142.29 & 4.35 \\
    \textbf{10} & \textbf{1000} &   43.65    & 37.29 & \underline{38.71} & 37.63 &  0.145     & \underline{0.123} & 0.094 & 0.092 & \underline{2}     & 282   & 4     & \underline{1.02}  & 141.98 & 2.04 \\
    \textbf{1000} & \textbf{10} &   43.99    & 38.60 & 38.40 & \underline{38.84} & 0.126      & \underline{0.100} & 0.056 & 0.066 & \underline{71}    & 282   & 267   & \underline{40.82} & 148.42 & 41.52 \\
    \textbf{1000} & \textbf{1000} &   44.37    & 39.06 & \underline{40.02} & 38.39 &  0.160     & \underline{0.123} & 0.092 & 0.091 & \underline{3}     & 282   & \underline{3} & \underline{1.04}  & 141.73 & 2.00 \\
    \hline
    \end{tabular}%
  \caption{The throughput (millions of queries/updates per second) with varied settings for three VM algorithms.}\label{tab:vmexp}%
\end{table*}%


\begin{figure*}
  \centering
  \begin{tabular}{ccc}
    % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
    \includegraphics[width=0.56\columnwidth]{../figures/max-version} & \includegraphics[width=0.56\columnwidth]{../figures/HP/max-version} & \includegraphics[width=0.84\columnwidth]{../figures/epoch/max-version} \\
    (a) Our wait-free algorithm (WF) & (b) Hazard-pointer (HP) & (c) Epoch (EP)\\
    \includegraphics[width=0.56\columnwidth]{../figures/ave-version} & \includegraphics[width=0.56\columnwidth]{../figures/HP/ave-version} & \includegraphics[width=0.84\columnwidth]{../figures/epoch/ave-version} \\
    (d) Our wait-free algorithm (WF) & (e) Hazard-pointer (HP) & (f) Epoch (EP)\\
  \end{tabular}
  \caption{The maximum number of live versions ((a)-(c)) and the average number of versions ((d)-(f)) for our wait-free algorithm (WF), a hazard-pointer-based algorithm (HZ) and an epoch-based algorithm (EP). For (b), the maximum number of versions stay the same (282) for all data pointers.}\label{fig:versions}
\end{figure*}




==> old/application.tex <==
\newcommand{\mm}{{\mathbb{M}}}
\hide{
\section{Implementations and Applications}
In this section we first show how to implement a persistent tree structure as the underlying data structure for our version maintenance problem, and then show two applications based on this implementation. For simplicity in implementations we only apply a lock-free but not wait-free algorithm in version control. We present two applications, which is a concurrent range sum and an inverted search index. In both applications we use one processor as the only writer, which incrementally add or remove entries to the current version and commit the result as a new version. At the same time we conduct $q$ concurrent queries at the same time. The reader, as well as the writer, may conduct operations modifying the tree, but only the writer can commit to the current version.

\subsection{Using a Persistent Tree as the Underlying Data Structure}
In this section we introduce how to implement a persistent balance tree structure as the underlying data structure for our algorithms. We note that this data structure has many good properties (functional, work-efficient, parallel, etc.) such that is can also be useful for other algorithms. We implement this data structure as part of a C++ library PAM \cite{pam}, with many highly-optimized parallel functions. We abstract the tree from the concrete balancing schemes. In PAM similar algorithms are applied on four balancing schemes: AVL trees, red-black trees, weight-balanced trees and treaps.

In each tree we store a set of key-value pairs, ordering by keys. It can also be augmented when necessary. Besides the tuple we also store the left and right children pointer, the size of the subtree, as well as a \emph{reference counter} (see details below). We access the tree by the pointer to the tree root. Each node in the tree can only be accessed following the path from a tree root to it.

\paragraph{Path-copying for Persistence.} In PAM persistence is supported by path-copying (or copy-on-write), which is a common technique widely used in many real-world systems~\cite{??} to support multi-version controlling. In PAM, any function that will effectively create a new tree will copy all the tree nodes on the update path. That is to say, every node that would be affected by this function (e.g., changing value or child pointer) will be copied and updated as a new node. Since the root is always on the update path, we can use the new root to represent the new tree. In this case all the untouched subtrees will be shared among trees. This guarantees that the extra space caused by a function is bounded by the work of the function. When multiple versions are alive, the total space is not necessarily the sum of all the trees, but can usually be much less due to nodes sharing.

\paragraph{Reference Counter GC.} Sharing nodes among trees can help save space when multiple version are alive, but may also cause problems when a tree is deleted, and the garbage collector should be able to tell which part is shared with other trees and keep them as is. To manage this we use the standard reference counting technique~\cite{Hudak86}. We store a reference counter in each tree node, which refers to the number of ``parents'' that have child pointers to it. When collecting a tree, we decrease the reference counter of the root node. If the counter decrease to 0, we free this node, and recursively decrease the counter of its two children. Otherwise the node is also in some other trees, so its children's reference counter does not change.  This is to guarantee that: 1) a node that is still in some alive version should never be collected and 2) a node that is not in any alive trees is collected.
The update on the reference counters are implemented by fetch-and-add.

\paragraph{Acquire and Commit to the Tree.}  To acquire a tree, we increase the counter of the root. The readers themselves can be parallel, modify the tree to answer queries and even keep multiple version in their local memory. We use the same algorithms with path-copying for readers and writers to modify the tree, but the readers just never commit to the current version.
For writers, to commit an updated version, it just changes the root pointer of the current version. If multiple writers are eligible to update the tree, this can be done with a compare-and-swap. This guarantees that all operations in a transaction, or all updates in a batch, appear in the current version atomically.

\paragraph{Optimization in Single-writer Version.} As mentioned in this paper we focus on the scenario that there is only one writer, in which case we can apply some optimizations to reduce the contention. Note that since our tree is purely functional, we never modify any data in the tree node (we copy and create new nodes), except the reference counter. Thus all contention occurs in updating the reference counters. Although never commit to the current version, the readers can modify the tree or do local garbage collection. This may cause update to the reference counters of the shared nodes, and further cause contention with the writer and other readers. To avoid this we keep a separate reference counter for the local computations of each reader, such that copying nodes in one processor will not affect others. When a reader is increasing the counter of a tree node $u$ in version $i$, and if $u$ is also visible to the outside world, we know $u$ will not be collected before the reader finishes. This is because $v$ is in at least a live version $i$. In that case, we do not need to increment the reference counter of $v$, and when doing local garbage collection, $v$ should not be collected as well. Thus, inside each reader processor, all updates in reference counters only occur in those nodes that are copied or created by this reader's local computation, which are invisible to any other processors. This means that there is no contention inside the tree structure.
}

==> old/functional.tex <==
\section{Functional Data Structures with Garbage Collection}
\label{sec:functional}

\guy{``functional'' in title is odd now that we moved the definition to preliminaries.   Perhaps this should just be dropped and the GC raised to a section.}

In this section, we show how to use an underlying functional data structure
to support our single-writer concurrency, and show an efficient \collect{}
algorithm for garbage collection with strong properties.
%
%
%\subsection{Multi-versioning Using Functional Data Structures}
%Using functional data structures gives an efficient solution for supporting
%multiple versions, since each update creates a new version while preserving the old one.

\guy{odd place for motivation of this sort.}

Using functional data structures for multi-versioning has several advantages. First,
any read or update can be done as if on a single-versioned system, oblivious to the existence of
other versions, since each update creates a new version while preserving the old one. This avoids the overhead of reading long version lists at each accessed node, which is common in other approaches to multi-versioning. Functional multi-versioning also allows for efficient GC with strong properties, as shown in the rest of this section.
%since much of the collection of one version is independent of the collection of another version.
% Also, as each version
%is a visible space from the version root, this allows efficient GC with strong properties.

%There can be many transactions with different versions simultaneously active.
%At any given configuration in a transactional history,
%the set of versions corresponding to active
%transactions form a set of roots into a memory graph.  These versions
%can share some of their tuples.

%\myparagraph{Garbage Collection.}



\begin{figure}%{r}{0.5\columnwidth}
     \vspace{-12pt}
     \begin{minipage}{.4\columnwidth}
       \framebox{\includegraphics[width=0.9\columnwidth]{../figures/persistence.pdf}}
     \end{minipage}
     \begin{minipage}{.5\columnwidth}
       \caption{{\small An example of the insert function under PLM using path copying. The output $T_2$ is represented by the root pointer at $5'$, while the input $T_1$ can still be represented by the original root pointer at $5$.
}\label{fig:persistence}}
     \end{minipage}
  
\end{figure} 


==> old/intro.tex <==
\section{Introduction}

Concurrent applications are designed to provide as much flexibility as
possible in the workloads that can be handled.  A lot of research has
gone into ensuring that data structures, transactional memories, and
other programs can guarantee safety and liveness, but often at the
cost of weak performance guarantees.  Although fully general, this
approach can overlook some real-world scenarios, where workloads are
better behaved, but good runtime guarantees are essential.
%However, for most real-world scenarios, conditions are better, and research focus can be .

An example of such a scenario is the case of online data services
involving heavy analytics on the data, but relatively light updates,
such as for web indices, social network graph databases,
%hybrid transactional/analytical processing (HTAP) databases,
or even
history of purchases.  In this scenario, it is essential that queries
can be executed quickly, concurrently, and with minimal delay, even if
they access large parts of the database.  Update operations may be
small or large, but happen continuously at a lower
throughput---for example a web crawler that updates the information
about pages as it crawls them.   In the scenario it can be acceptable
to sequentialize the updates, or the updates are simple enough that
they can be batched and processed as parallel bulk updates.

%\renewcommand{\thefootnote}{\fnsymbol{footnote}}
%\footnotetext[1]{We submit a full version of this paper in the supplement material with all proofs and discussions of this paper.}
%\renewcommand*{\thefootnote}{\arabic{footnote}}

%\Yihan{may want to mention that there are real-world database systems like CouchDB \cite{couchdb} that guarantee serializability by batching concurrent updates and executing them by a single writer.}

In this paper, we consider a setting that performs especially well in
such conditions.  More specifically, we study \emph{single-writer
  concurrency}, where many read transactions, but just one write
transaction, can be concurrent at any time.  In this setting, we design
a transactional memory in which transactions never abort and execute
in a number of steps that can be tightly bounded, and for which
garbage collection is safe and precise.  While some of these
properties can be achieved with multiple writers, we know of no
previous transactional memory system that achieves these properties
simultaneously, even when restricted to single-writer executions.

\lstset{basicstyle=\footnotesize\ttfamily, tabsize=1, escapeinside={@}{@}}
\lstset{literate={<<}{{$\langle$}}1  {>>}{{$\rangle$}}1}
\lstset{language=C, morekeywords={CAS,commit,empty,local,job,taken,entry,GOTO}}
\lstset{xleftmargin=5.0ex, numbers=left, numberblanklines=false, frame=single}
%\lstset{caption={\texttt{tuple} and \collect{} algorithms},captionpos=b,label={alg:collect}}
%% \makeatletter
%% \lst@Key{countblanklines}{true}[t]%
%% {\lstKV@SetIf{#1}\lst@ifcountblanklines}

%% \lst@AddToHook{OnEmptyLine}{%
%% 	\lst@ifnumberblanklines\else%
%% 	\lst@ifcountblanklines\else%
%% 	\advance\c@lstnumber-\@ne\relax%
%% 	\fi%
%% 	\fi}
%% \makeatother

\begin{figure*}\small
\begin{minipage}{.49\textwidth}
\begin{lstlisting}
v = acquire(k);  //@\phaseone@
user_code(v);		  	//@\phasetwo@
// Can respond to user here
res = release(k);	//@\phasethree@
if (res) {			   	//@\phasefour@
  collect(v);	}		
  
\end{lstlisting}
\centering Read Transaction
\end{minipage}~~~
\begin{minipage}{0.49\textwidth}
\begin{lstlisting}
v = acquire(k);     //@\phaseone@
newv = user_code(v);	//@\phasetwo@
flag = set(newv);				  //@\phasethree@
// Version visible here
res = release(k);	
if (res) {					//@\phasefour@
  collect(v);	}
//if flag is false, retry or abort
\end{lstlisting}
\centering Write Transaction
\end{minipage}
\vspace*{-.1in}
\caption{Transaction Phases. $k$ is the process ID.}
\vspace*{-.1in}
\label{alg:framework}
\end{figure*}

Our approach is based on
multiversioning~\cite{Reed78,BG83,papadimitriou1984concurrency,perelman2010maintaining,Kumar14}.  It, however, avoids version lists
\cite{Reed78,BG83,papadimitriou1984concurrency,Kumar14,neumann2015fast}, since
they can cause delay to access data, and can cause difficulties for
garbage collection.
% allowing the readers to proceed without delaying or aborting the
%writer, and the writer to proceed without delaying or aborting the
% readers.
%A key feature of our design is that we create a multiversioned
%transactional memory, but maintaining many such versions does not
%translate to increased complexity in steps or space.
%% A common approach to multiversioning is to maintain a ``history'' of
%% versions of each object as a timestamped linked list, and have each
%% transaction traverse the version list at every object of the database to find
%% the right version
%% \cite{Reed78,BG83,papadimitriou1984concurrency,Kumar14}. This means
%% that transactions spend a significant amount of effort traversing
%% these lists, even if the database itself is small.  It also
%% complicates garbage collection since information about a particular
%% version can be spread throughout the version lists.  We give a more
%% detailed overview of the related work in Section \ref{sec:related}.
Instead we use two key ideas: (1) a
solution to which we refer as the \VerMain{} problem for the purpose
of acquiring, releasing and creating a new version, and (2) functional data
structures~\cite{Okasaki98,BenAmram95,KT96,Pippenger97},\footnote{This
  is the style used in all functional languages, including Haskell,
  OCaml, ML, and F\#, and is often also used in imperative languages
  for safety or to maintain persistent copies of data.}
%The style is
%  well suited for pointer based structures such as trees, but has an
%  $O(\log n)$ overhead for updating arrays.}
for the purpose of
making fast ``copies'' without side effects, and an associated garbage
collection algorithm.  We assume each version is organized as a DAG
which can be accessed by a single entry node (e.g., a tree accessed by
its root), and that the DAG cannot be side-effected (it needs to be
persistent~\cite{driscoll1989making}).

The \VerMain{} problem supports three operations.  The \acquire{}
operation, acquires the current version (i.e., the entry node for the
version), the \release{} operation releases the version grabbed by
the corresponding \acquire{}, and
returns a flag indicating whether this is the last usage of this
version, and the \set{} operation sets a new current
version by supplying a new entry node.
Figure~\ref{alg:framework} illustrates how these can be used in read
and write transactions.  A valid solution to the \VerMain{} problem
must guarantee it is safe to collect a version if the \release{}
returns true.  We describe a wait-free algorithm for the \VerMain{}
problem.
%% We design the wait-free algorithm carefully to ensure that it
%% will never suffer from high contention costs. That is, we prove that
%% regardless of the workload, as long as there can only be one active
%% \set[] operation at any time, the contention experienced by any
%% process is bounded to an amortized constant amount per step.
We show that the \acquire[] operation requires only a constant number of
steps, and thus beginning a transaction incurs almost no delay.
We also show that the operations have low memory contention.  We expect that the \VerMain{} problem and our algorithms are general enough to be of independent interest.

 %% In the \emph{\phaseone}, each transaction calls \acquire[] to obtain a version $v$ (ideally the most recent version). Then in the \emph{\phasetwo{}}, the user code is executed on $v$. The response to a read transaction is ready at this point. The \emph{\phasethree{}} starts when the user code terminates. The write transaction first calls \set[] to commit a new version, after which the new version is visible to the outside world. Then all transactions call \release[] to signal that this process is no longer using the version, and return \true{} if and only if it is the last processor working on this version, in which case, this version is then garbage collected in the \emph{\phasefour{}}.
%Finally, \emph{\phasefour{}} works on GC if if the \release() \op{} returns \true.
%Finally, \emph{\phasefour{}} works on GC if necessary: if the \release() \op{} returns \true, then the \texttt{collect}($v$) function is called in order to garbage collect the version.
%A transaction's invocation is defined as the beginning of the \phaseone, and its response is at the end of the \phasefour. The transaction is \activet{} for the entire interval between its invocation and response.

%% Our approach consists of two parts; the first, referred to as the \VerMain{} problem, deals with the \phaseone{} and \phasethree{}, and the second handles the garbage collection.
%% %The first part deals with the \phaseone{} and \phasethree{}, and is based on what we refer to as the \VerMain{} problem.
%% The \VerMain{} problem aims at maintaining versions of a database in a way that allows quick access to active versions and easily identifies outdated ones. More specifically, a version maintenance object supports three operations: \acquire{}, \release{}, and \set{} on a concurrent data structure.

%Any transaction must begin by calling \acquire{} in order to gain access to the most recent version, and must call \release{} before terminating to signal that it is no longer using the version. An write transaction calls \set{} in order to update the current version. The \release{} operation returns \true{} if and only if no transaction will ever use the newly released version again, thus indicating that it is safe to collect. Figure~\ref{alg:framework} shows how we use the VM object in our transactional framework. However, we believe that the VM problem is general enough to be of independent interest.

Functional data structures allow for fast ``copying'' of DAG structures
using path copying \cite{Okasaki98}.
%% copying old data can be quite efficient %, both in time and space, by
%% by path copying \cite{Okasaki98}.
%% To make the versions persistent requires ``copying'' the DAG.  In
%% general this could be expensive, but using
With path copying, only nodes on the update path are copied and most of
the DAG can be shared among versions (see Figure \ref{fig:persistence}
as an example).  Furthermore, the cost of traversing a data structure
is independent of the number of versions and requires no synchronization, unlike version lists.
%% For
%% example, even considering an unbounded number of versions, the number
%% of steps taken by a transaction that finds a key in a balanced tree
%% is $O(\log n)$.
%, and an insertion on a balanced tree which yields a new
%version also requires $O(\log n)$ steps
%The second part of our framework is a \collect{} algorithm for GC, which is \phasefour{} in our transactional memory.
% Also garbage collection can be handled using reference
% counting.
We describe a \collect{} algorithm based on reference counting and
show it is safe (all freed nodes are out-of-date),
precise (all out-of-date nodes are freed),
and efficient (strong time bounds)---definitions in Section
\ref{sec:gc}.
Our garbage collection conditions are similar to
the UP-GC condition~\cite{perelman2010maintaining}.
%considered Perelman et. al.
Functional data structures work particularly well with the \VerMain{} problem
since the entry node of the DAG can be used to represent data,
and as the value to be acquired, set, and collected.
\begin{table}
  \centering
  \small
  \begin{center}
  \begin{tabular*}{\linewidth}{c||r|c@{ }c@{ }||@{}c@{}}
    \hhline{-----}
    &\multicolumn{3}{c||}{\textbf{Time Bound}} & \textbf{Properties}\\
\hhline{=====}
    & \multicolumn{3}{@{}c||}{Thm. \ref{thm:waitfree-step} and \ref{thm:contention}} &Thm. \ref{thm:waitfree-lin}\\
\cline{2-5}
    \textbf{} & &    \textbf{Steps}&\textbf{Contention} & No abort and wait-free\\
\cline{2-4}
    \textbf{VM}&\textbf{\acquire{}} & $O(1)$& $O(1)$& for readers and one writer,\\
    %\cline{2-4}
    \textbf{}&\textbf{\release{}} & $O(P)$& $O(P)$&linearizable\\
    %\cline{2-4}
    &\textbf{\set{}} & $O(P)$& $O(P)$&\\
    \hhline{=====}
    \multirow{2}{*}{\textbf{GC}}&\multicolumn{4}{c}{Thm. \ref{thm:collect-correct}}\\
    \cline{2-5}
     & \multicolumn{3}{c||}{$O(S+1)$ steps} & Safe and precise\\
     %\cline{1-5}
    %\hline\hline
     \hhline{=====}
    &\multicolumn{3}{@{}c@{}||}{Thm. \ref{thm:waitfree-step}, \ref{thm:contention} and \ref{thm:collect-correct}}& Thm. \ref{thm:serial} and \ref{thm:safe-precise}\\
    \cline{2-5}
 \textbf{In} & \textbf{Reader}& \multicolumn{2}{c||}{delay-free} & No abort and wait-free \\
    %\cline{2-4}
 \textbf{All}   & \textbf{Writer} &\multicolumn{2}{c||}{$O(P)$-delay}&  for readers and one writer,\\
        %\cline{2-4}
    &\textbf{GC} & \multicolumn{2}{c||}{$O(S+1)$ steps}&serializable, safe and precise GC\\
\hhline{-----}
  \end{tabular*}
  \end{center}
  \caption{\small The time bounds and properties guaranteed by our algorithms and the corresponding theorems in this paper. ``VM'' means the \VerMain{} problem. $P$ is the number of processes. The contention bounds are amortized. In GC, $S$ is the number of tuples that were freed. ``Delay'' is defined in Section 2. Safe and precise GC are defined in Section \ref{sec:gc}. }\label{tab:allresults}
  \vspace{-.25in}
\end{table}


\hide{
A key feature of our design is that we create a multiversioned transactional memory, but maintaining many such versions does not translate to increased step complexity.
A common approach to multiversioning is to maintain a `history' of each node's versions, as a timestamped linked list, and have each transaction traverse the list at every node of the database to find the right version \cite{overmars1983searching,and,more}. This means that transactions spend a significant amount of effort traversing these lists, even if the database itself is small.
Our algorithm gets around that, by combining the version maintenance object with an underlying functional database \cite{Okasaki98,BenAmram95,KT96,Pippenger97}\footnote{This is
	the style used in all functional languages, including Haskell,
	OCaml, ML, and F\#, and is often also used in imperative languages
	for safety or to maintain persistent copies of data.  The style is
	well suited for pointer based structures such as trees, but has an
	$O(\log n)$ overhead for updating arrays.}. That is, rather than modify the value at any node and create a linked list of old versions, an updating transaction instead makes a copy of the old data, with the desired updates, and simply swings the `head' pointer to point to the root of the new copy. Using path copying \cite{Okasaki98}, this technique can be quite efficient.
In this way, the size of the data structure that any transaction must traverse is exactly the size it would be if there were only one version. This allows us to bound the work of a transaction by the work it would have done sequentially; for example, bounding the number of steps taken by a transaction that finds a key in
a balanced tree to $O(\log n)$ steps. More formally, we define \emph{delay} as the number of \emph{extra} steps a transaction must take on top of what it would have if it were to execute in isolation on a single-versioned system. We say that a transaction is \emph{delay-free} if its delay is a constant.
As far as we know, ours is the first multiversioned transactional system to allow for the transactions' user-code to be delay-free.}
%
%\begin{wrapfigure}{r}{3.4in}
%\begin{figure}
%  \begin{center}
%     %\vspace{-.3in}
%    \framebox{\includegraphics[width=0.9\columnwidth]{../figures/transtimeline}}
%  \end{center}
%  \vspace{-.1in}
%  \caption{{\small A time line for transactions manipulating a balanced
%    tree of size $n$.  User code is marked in gray.  $v_a$ and $v_b$
%    are versions of the tree before and after inserting $y$.  The
%    values at the top are the values returned by \acquire{} (AQ) and
%    \release.  The big-O bounds are upper bounds on step counts.
%    $|v_a\backslash v_b|$ indicates the number of nodes in $v_a$ but
%    not $v_b$. GC means garbage collect.}}
%  \label{fig:transtimeline}
%\end{figure}
%\end{wrapfigure}

%% roughly speaking
%% the delay is the number of \emph{extra} steps a transaction must take on top of what it would have if it were to execute in isolation on a single-versioned system.  We say that a transaction is \emph{delay-free} if its delay is a constant.
%% As far as we know, ours is the first multi-versioned transactional system to allow for the transactions' user-code to be delay-free.
%In summary, our transactional memory system achieves the following properties, which are also summarized in Table \ref{
%\Naama{Haven't talked about the `phases' that we use in the following list.}

%% \begin{enumerate}[itemsep=0pt]
%% \item
%% All transactions are strictly serializable and none ever aborts.  This by
%% itself is achieved by many previous multiversioning approaches when
%% there is a single writer. %(Proved by Theorem \ref{thm:serial})
%% \item
%% A read-only transaction is delay-free until after it responds to the user.
%% %The \acquire{} takes a constant number of steps in the worst
%% %case, and has constant contention in the amortized case. (Proved by Theorem \ref{thm:waitfree-time})
%% %\item
%% %If the user transaction takes $s$ steps sequentially, then the
%% %\phasetwo{} takes $O(s)$ steps, and the \phasetwo{} of a read transaction
%% %experiences no contention. (Can be seen from Figure \ref{alg:framework} and Observation \ref{no-contention})
%% \item
%% A write transaction has an additive delay of $O(P)$ steps before its version is committed.
%% %\item
%% %
%% %  The \set{} and \release{} take at most $O(P)$ steps and with $O(P)$
%% %  amortized contention. (Proved by Theorem \ref{thm:waitfree-time})
%% \item
%% All transactions incur $O(P)$ delay when releasing a version.
%% \item
%%   If there are $W$ write transactions allocating a total of $S$ space then the total steps
%%   across all \phasefour{}s is at most $O(W+S)$ %(Proved by Theorem \ref{thm:collect-correct})
%%   %---i.e. collection takes linear steps in what needs to be collected.
%% \item
%% The garbage collection is precise in that it never holds onto any
%% versions that are not the latest version, or held by an active
%% transaction.  This is similar to the UP-GC condition considered
%% Perelman et. al.~\cite{perelman2010maintaining}. It is also safe, never freeing a \tuple{} that may be accessed in the future. %(Proved by Theorem \ref{thm:safe-precise})
%% \end{enumerate}

Our results are summarized in Table~\ref{tab:allresults} and described
in sections~\ref{sec:vermain}, \ref{sec:gc} and \ref{sec:setup}.
%An example is given in Figure~\ref{fig:transtimeline}, assuming an underlying functional balanced tree structure.
%Delay is defined in Section~\ref{sec:prelim}, and is stronger than wait-free.
One concern with having a single writer is that it could limit the
update throughput.  However, assuming that the updates can be
batched~\cite{postgressnapshot,palm,hendler2010flat,batcher}---simple to do for inserts or deletes, for example---then the
system can accumulate updates over time and process them in parallel
at regular intervals, committing in bulk.   This makes
an update transaction atomic without any locking, which is hard for most
concurrent structures
%For example, a new document can be added to the inverted index atomically (consisting of thousands term updates).
(discussed in Section~\ref{sec:batching} and \ref{sec:exp}).

To test the efficacy of our approach we implemented our wait-free
algorithm for the \VerMain{} problem and use the functional tree
structure.  We test the performance
of functional tree structure with a single writer and batched updates
both on an ordered dictionary and an inverted index.
Our experiments show that our implementation outperforms many
state-of-the-art concurrent data structures even with a single writer,
and that the update and queries do not delay each other.
We also combine our wait-free algorithm with the functional tree structure,
and test them under different conditions. Experiments show that our wait-free
algorithm collects old versions fairly timely, and suffers from little contention
between threads. Also, the overhead of introducing
both a single writer and GC is reasonably small.

We submit a full version of this paper with all proofs and discussions in the supplemental material.

%To test the efficacy of our approach we implemented our wait-free
%algorithm for the \VerMain{} problem and tested on two test cases.
%For the functional data structures we use the PAM library~\cite{pam},
%which supports functional trees in C++.  The first test case is for
%maintaining an ordered dictionary, supporting insertions, deletions
%and searches.  We show a variety of experiments on different batch
%sizes, and compare to state-of-the-art concurrent dictionaries, where
%in most cases we perform the best.  The second test case is for
%maintaining a document index supporting insertion/deletion of
%documents, and logical queries over terms (reporting all documents
%that match the query).  In this case the operations are coarser
%grain---a document insertion could insert entries for many thousands
%of terms, and queries have to go over large posting lists of documents
%containing the given terms.  We show that the concurrent insertions
%does not significantly effect the performance of queries.  An
%important advantage of our structure over using a concurrent tree is
%that a document can be added atomically (consisting of thousands term
%updates) without any locking.


%% The rest of the paper is organized as follows. In Section \ref{sec:prelim}, we go over our model and some basic definitions. Then, in Section \ref{sec:vermain} we formally present the version maintenance problem and give an efficient wait-free algorithm for it. In Section \ref{sec:gc}, we briefly discuss garbage collecting in our functional version framework, and then bring these elements together to form our transactional memory system in Section \ref{sec:setup}. At the end of the paper, we discuss related work (Section \ref{sec:related}), and conclude with some discussion of extensions to our work in Section \ref{sec:discussion}.
%% Due to space limitations, we put the full version of the paper in the supplement material, which includes full proofs of correctness and efficiency for our version maintenance algorithm and garbage collection, as well as more experimental results.

%%%%%%%% I think we might not actually need the figure. At least for the intro as it is right now, it doesn't add much %%%%%%%%
%
%\begin{wrapfigure}{r}{3.4in}
%	\begin{center}
%		\vspace{-.3in}
%		\framebox{\includegraphics[width=0.50\columnwidth]{../figures/transtimeline}}
%	\end{center}
%	\vspace{-.25in}
%	\caption{\small A timeline for transactions manipulating a balanced
%		tree of size $n$.  User code is marked in gray.  $v_a$ and $v_b$
%		are versions of the tree before and after inserting $y$.  The
%		values at the top are the values returned by \acquire{} (AQ) and
%		\release.  The big-O bounds are upper bounds on step counts.
%		$|v_a\backslash v_b|$ indicates the number of nodes in $v_a$ but
%		not $v_b$. GC means garbage collect.
%		\vspace{-.2in}}
%	\label{fig:transtimeline}
%\end{wrapfigure}
%
%
%Figure~\ref{fig:transtimeline} gives an example of the interleaving
%for insertion and finding a key in a balanced tree.  An important
%property is that the \textbf{find} in the queries is finished and can
%be reported in the optimal $O(\log n)$ steps.  For all but the \phasefour
%and writer transactions the only synchronization instruction we need
%is a CAS.  For the \phasefour and for the writer we use a
%fetch-and-add to support reference counting garbage collection.  Other
%schemes for maintaining a counter could be used instead, to avoid the
%use of fetch-and-add, and to potentially improve
%performance~\cite{acar2017contention,ellen2007snzi,herlihy1991wait}.
\hide{
\begin{table}
  \centering
  \begin{tabular}{|c|ll|c|}
    \hline
    &\multicolumn{2}{c|}{\textbf{Delay}}&\textbf{Contention}\\
    \hline
    \textbf{\acquire{}} & \multicolumn{2}{c|}{$O(1)$}& $O(1)$\\
    \hline
    \textbf{\release{}} & \multicolumn{2}{c|}{$O(P)$} & $O(P)$\\
    \hline
    \textbf{\set{}} & \multicolumn{2}{c|}{$O(P)$}&$O(P)$\\
    \hline
    \hline
    &\multicolumn{2}{c|}{\textbf{Time bound}} & \textbf{Properties}\\
    \hline
    \textbf{VMP Algorithm} & \multicolumn{2}{c|}{as shown above} & no abort, linearizable\\
    \hline
    \textbf{GC} & \multicolumn{2}{c|}{$O(W+S)$} & Safe and precise\\
    \hline
    \multirow{2}{*}{\textbf{In all}} & read txns:& delay-free & no abort, serializable, wait-free,\\
    \cline{2-3}
    & write txns: &$O(P)$-delay& low delay, safe and precise GC\\
    \hline
  \end{tabular}
  \caption{A}\label{tab:all}
\end{table}
}



==> old/lockfree.tex <==
%\subsection{A Lock-free Algorithm}
%\label{sec:lockfree}

\newcommand{\current}{{\texttt{cur\_idx}}}
\newcommand{\version}{{\texttt{version}}}
\newcommand{\info}{{\texttt{info}}}
\newcommand{\datastructure}{{\texttt{data}}}
\renewcommand{\figurename}{Algorithm}
\lstset{basicstyle=\footnotesize\ttfamily, tabsize=2, escapeinside={@}{@}}
\lstset{literate={<}{{$\langle$}}1  {>}{{$\rangle$}}1}
\lstset{language=C, morekeywords={CAS,commit,empty,local,job,taken,entry,GOTO}}
\lstset{xleftmargin=5.0ex, numbers=left, numberblanklines=false, frame=single}
%\lstset{caption={Lock-free algorithm for the Version Maintenance Problem},captionpos=b,label={alg:lockfree}}
\begin{figure}
	\caption{Lock-free algorithm for the Version Maintenance Problem}
\begin{lstlisting}[countblanklines=false]
struct Version{ int timestamp; 	int index; };
struct VersionStatus{ Version v; int count; };
Version V;
VersionStatus S[2*P];
Data* D[2*P];
Version empty = <-1, -1>;
Version A[P]; //Persistent local vars.

Data* acquire(int k) {
  Version v, VersionStatus s;
  do { v = V;@\label{line:lockfree_acquire_get}@
    s = S[v.index];
  } while (!CAS(S[v.index],   @\label{line:lockfree_acquire_CAS1}@
    <v,s.count>, <v,s.count+1>));
  A[k] = v;
  return D[v.index]; }

bool release(int k) {
  Version v = A[k]; bool last = false;
  do { VersionStatus s = S[v.index];
    if(s.count == 1) last = true;
  }while (!CAS(S[v.index],s,<s.v,s.count-1>));@\label{line:lockfree_release_CAS}@
  if (v == V || !last) return false; @\label{line:lockfree_release_condition}@
  VersionStatus s = S[v.index];
  if(s.v != <v, 0>) return false;@\label{line:lockfree_gc_abort}@
  return CAS(S[v.index],s,<empty,0>); }@\label{line:lockfree_gc_CAS}@

void set(Data* d) {
  int index = random_hash(0, 2*p);
  while (S[index] != <empty, 0>) {
    index = (index+1)%(2*p); }
  Version v = <V.timestamp+1, index>;
  S[index] = <v, 0>; @\label{line:lockfree_ws}@
  D[index] = d; V = v; }
\end{lstlisting}
\vspace{-.3in}
\label{alg:lockfree}
\end{figure}
\renewcommand{\figurename}{Figure}
\putmaybeappendix{lockfree-algo}
\begin{maybeappendix}{lockfree-algo}

In this section, we describe our lock-free algorithm for version maintenance.
The algorithm uses a hash table $S$ to maintain the status of all live versions. Similarly, a hash table $D$ is used to store the data pointers associated with the live versions. Each non-empty element of $S$ stores a version along with the count of that version. Intuitively, the count of each version represents the number of processes working on that version. We represent a version $v$ as a timestamp plus an index. The index tells us which element of $D$ and $S$ is reserved for that version. \texttt{A} is an announcement array mapping each processor id to the version it is working on.
%We use hash tables to maintain information on all live versions.
Note that at any time, there can be at most $P$ live versions, so both hash tables have size $2P$. We use a global variable \currentv{} to represent the current version.
%\Naama{$v$ isn't a good notation for a hash table. Can we use something like $\mathcal{H}$ instead?}
%\HAO{I changed the notation to $S$ for version status and $D$ for data pointer. This is consistent with our waitfree algorithm. Maybe calling them $\mathcal{H}$ and $D$ might make sense too.}
%Each entry in the hash table consists of two parts, a pointer to the data structure, \datastructure{} and some extra information \info{}.
%\Naama{is \datastructure{} the data structure itself, or is it the pointer to it? If it is the latter, what is the different between \datastructure{} and \texttt{root}?}
%The \info{} is a pair of a integer \emph{version number}, and an integer \emph{counter} recording the number of processors that is working on this version. The version number is a globally maintained number assigned to each version, and is $-1$ if the this version is not valid.
%The global variable \currentv{} is used to store the current version.
%We use an integer \current{} to denote the index of the current version in $v$, and \version{} to denote the time stamp, which is the total number of versions that ever lived. We assume the underlying data in \datastructure{} can be accessed by a pointer \texttt{root}. Any update or garbage collection will directly operate on this root.

\myparagraph{Acquire.} The acquire operation reads the most recent version from $V$, increments the count of that version, and returns the data pointer associated with it. Incrementing the counter is implemented by performing a CAS in a loop. Every time the CAS fails, the operation re-reads the current version and the status of that version.
% Since the status of a version contains the timestamp of that version, there cannot be any ABA problems.
Before returning, an \acquire($k$) operation writes the version that it acquired into its persistent local variable $A[k]$. This is so that the next call to \release($k$) knows which version to release.
%make sure this is the current version.
%Note that the version number $i$ that a processor $p$ acquires is not necessarily the current version (except for the acquire of the writer, which will always return the current version) when it returns, but is still a valid version whose counter value is greater than 0, so that it will not be collected by others before $p$ terminates.

%\paragraph{Find.} This operation finds an empty slot in the hash table $S$. It is done by choosing a random index and doing linear probing.

\myparagraph{Set.} %After the writer updates a new version, it will call the \set{} operation to commit.
The \set($d$) function first randomly finds an empty slot \texttt{i} for the new version in the hash table $S$.
% (the hash table is accessed using linear probing)
Then it creates a new version $v$ using index \texttt{i} and the current timestamp plus one. Then it stores $v$ into $S[i]$ with count $0$. Finally, it writes $d$ into $D[i]$ and sets $v$ as the current version.
% Then it sets the \datastructure{} in $v[i]$ as the updated data structure. The corresponding version number is set to be the current time stamp plus one.
%Finally, we update \current{} to $i$.
%The order matters since whenever the \current{} is acquired by other threads, the whole version must be ready, and whenever the flag is read as \texttt{true}, the data structure should be ready.

\myparagraph{Release.} Basically, a \release($k$) operation decrements the counter of the corresponding version \texttt{v}, and collect the corresponding version if necessary. Intuitively the \release{} function returns true iff it does the garbage collection of its corresponding version (will be proved later).
The \release($k$) operation first reads $A[k]$ to check which version it's responsible for decrementing.
%In our algorithm, the last one that releases this version is always responsible to collect it.
Then it tries to decrement the counter with a CAS, just like an \acquire{} operation, retrying until successful. After the decrement, if $v$ is still the current version or if the count of $v$ is non-zero then the operation returns \false{} because $v$ is still live. Otherwise, the count of $v$ is 0 and $v$ is no longer the current version, so the \release($k$) operation tries to make $v$ unacquireable by setting $S[v.index]$ to empty with a CAS. If it succeeds, then $v$ is no longer live and it returns \true{}. Otherwise, either some other operation has set $S[v.index]$ to empty or some \acquire{} operation has incremented the count of $v$. In the first case, the \release($k$) operation returns \false{} because some other \release[v] operation has already returned \true{}. It also returns \false{} in the second case because $v$ is still live.
%we know this may be the last one leaving this version. In this case, it is this processor's responsibility to collect the version, unless this version is still the current version.

% If the released version needs to be collected, we check again this version is still with version \texttt{v} and count 0, then use a CAS to swap in the \texttt{empty} version. If the last CAS fails, it means that the collection is done successfully by some other threads.
%A processor $p$ will collect a version $v$ after releasing if and only if $v$ is not the current version and $p$ is the last one working on $v$.
%This is safe because if this is not the current version, there will never be new readers accessing this version again.

%One thing to note here is that, since we never collect the current version, when all the readers left the current version, it should still stay alive. This may cause problem when the writer updated a new version, and the old version will be left as garbage. As a result we may run out of space in the hash table. We address this problem in the \texttt{find} function. Each time we execute the linear probing, if we see a version that is not the current version, but has reference counter 0, we collect it, and return this slot. It is safe because since it is not the current version, it will not be read by any readers then.


%\paragraph{GC.} This function collects an out-of-date version $v[i]$ in the hash table, with version number $V$. It first saves the pointer of \datastructure{} in $v[i]$ and the current \info{} of $v[i]$ as $x$.
%We further check if now $x$'s version number is no longer $V$, or its count is more than 0, we abort.
%We use a CAS to set the version number and counter to $\langle -1,0\rangle$. From this point, this slot in the hash table is available for the writer to use for a new version, even though the data in \datastructure{} might not have been collected yet. It then calls the garbage collector of the corresponding data structure on the old pointer of \datastructure{}.
% \Naama{Can we merge the GC function with the release? That way, it matches up with the wait-free algorithm better. I also think it can save us a bit of space, since we don't need all of this description.
%	We discuss how to use the version maintenance for actual garbage collection in a different version, so i think it's ok if we leave it out here.}

% \HAO{I added the array A so that there would be a way of communicating the acquired version to the release operation.}

% \Naama{The pseudocode uses different notation than the text that talks about it. We need to fix that. In particular, the text uses $v$ to refer to the hash table, which I think is bad notation anyway.
% I think the hash table in the code is D, or type VersionDataD? But it doesn't correspond to the struct name defined above it. And in any case, I think we should rename it to make it clear that this is a hash table.}
\end{maybeappendix}

%\myparagraph{Correctness.}
%\subsection{The Correctness of the Lock-free Algorithm}
\begin{maybeappendix}{lockfree-correctness}
In this section, we show that our lock-free algorithm is linearizable. The result can be summarized as Theorem \ref{thm:lockfree-lin}. We defer the full proof to the supplement material.

\begin{theorem}\label{thm:lockfree-lin}
    Algorithm \ref{alg:lockfree} is a linearizable solution to the Version Maintenance problem.
\end{theorem}

We first present the linearization points for each operation in our lock-free algorithm.

\begin{definition}\label{def:lf_linpoint}
  For each \op{} $op$, its \emph{linearization point} is as follows:
  \begin{itemize}
    \item If $op$ is a \set[], then it is linearized at line \ref{line:lockfree_ws}. This is the line that updates \currentv{}.
    \item If $op$ is an \acquire[], then it is linearized on line \ref{line:lockfree_acquire_get} of the loop that performs a successful CAS on line \ref{line:lockfree_acquire_CAS1}.
    \item If $op$ is a \release{}, then there are two cases:
      (1) If $op$ completes and returns \true, then it is linearized at its final step.
      (2) Otherwise, it is linearized when it performs a successful CAS on line \ref{line:lockfree_release_condition}.
  \end{itemize}
\end{definition}

In the supplement material we then prove that these linearization points satisfy the sequential specification outlined in Section \ref{sec:prop-proof}, which them proves Theorem \ref{thm:lockfree-lin}.

However note that this algorithm is not wait-free, and does not have time bounds. In particular, the while loop in \acquire{} can run arbitrary long. This is because of the infinite loop in updating counters.
Nevertheless, in the experiment we will show that this algorithm can work well in practice, and is especially easy to implement. In the supplement material, we also show an efficient wait-free algorithm for the \VerMain{} problem.


%\noindent \textbf{Linearization points}:
%\begin{itemize}
%  \item Acquire(): At the point to get the current version (Line \ref{line:lockfree_acquire_get}) in the loop of the successful CAS .
%  \item Set(): When it set the current version to be the new version.
%  \item Release(): For those returning \false{}, the point is set to the point when CAS succeed. For the \release{} returning \true{}, it is at the point where \gc{} returns \true{}.
%\end{itemize}



We refer to $S[v.index]$ as the counter of $v$. Intuitively, \release{} operations returning \false{} are linearized when they decrement the counter of the version they are trying to release.
%Also, we linearize \acquire{} operations at when it reads the version whose count it will eventually increment on line \ref{line:lockfree_acquire_CAS1}.
Also, we linearize \acquire{} operations at when it reads the version it later successfully grabs.
We first prove the following two helper lemmas for better understanding the algorithm.

\begin{lemma}
\label{lem:lf_live}
When the counter of a version $v$ is more than 0, this version is live.
\end{lemma}

\begin{proof}
The counter of a version $v$ is more than 0 only if line \ref{line:lockfree_acquire_CAS1} of an \acquire[v] operation increments the counter and the counter has not yet been decremented by line \ref{line:lockfree_release_CAS} of the corresponding \release[v] operation. Since \acquire[v] operations are linearized before they increment the counter and \release[v] operations are linearized either when they decrement the counter or at some later step, we know that $v$ is live whenever its counter is more than 0.
\end{proof}

\begin{lemma}
\label{lem:lf_unique}
For each version $v$, there is at most one \release[v] operation that returns \true{}.
\end{lemma}

\begin{proof}
A \release[v] operation returns \true{} only if the CAS on line \ref{line:lockfree_gc_CAS} changes $S[v.index]$ from $\langle v, 0\rangle$ to $\langle empty, 0\rangle$. The lemma holds because $S[v.index]$ will never change back to $\langle v, 0\rangle$ after it has been set to $\langle empty, 0\rangle$.
%\HAO{more justification needed here}
%To prove the lemma, it suffices to show that $S[v.index]$ will never be changed back to $\langle v, 0\rangle$.
%The only instructions that write to $S$ are on lines \ref{line:lockfree_ws}, \ref{line:lockfree_release_CAS} and \ref{line:lockfree_acquire_CAS}. \set() operations always write newer versions to $S$, so line \ref{line:lockfree_ws} will not set $S[v.index]$ back to $\langle v, 0\rangle$. The CAS on line \ref{line:lockfree_release_CAS} cannot succeed as long as
\end{proof}

Now we are ready to show that the linearization points satisfy the sequential specifications. Lemma \ref{lem:lockfree-acquire} proves the first part of the sequential specifications, which says that \acquire() operations return the correct value. Together, Lemmas \ref{lem:lockfree-1} and \ref{lem:lockfree-2} prove the second part of the sequential specification, which says that a \release[v]() operation returns 1 if and only if $v$ changes from being live to not live.

\begin{lemma}
\label{lem:lockfree-acquire}
An \acquire(k) \op{} $Q$ returns the pointer written by the last \set() \op{} linearized before it.
%It will still stay live when \acquire{} returns.
\end{lemma}

\begin{proof}
Note that at any point in an execution, the global variable \currentv{} stores the \vptr{} created by the last \set() operation linearized before this point. Furthermore, at any point in the execution, $D[\currentv{}.index]$ stores the pointer written by the last \set() \op{} linearized before this point. This is because $D[i]$ cannot change as long as $S[v.index] \neq \langle empty, 0\rangle $ and $S[v.index]$ cannot be set to $\langle empty, 0\rangle $ as long as $i = \currentv{}.index$ (due to the check on line \ref{line:lockfree_release_condition}).

Let $v_0$ be the value of \currentv{} at $Q$'s linearization point. It's easy to see that $Q$ increments the count of $v_0$ by looking at how \acquire{} operations are linearized. While the count of $v_0$ is non-zero, $S[v_0.index]$ cannot be set to $\langle empty, 0\rangle $ because the CAS on line \ref{line:lockfree_gc_CAS} of \release[v_0] only succeeds when the count of $v_0$ is zero. Therefore $D[v_0.index]$ cannot be changed as long as the count of $v_0$ is non-zero, so $Q$ returns the data pointer associated with $v_0$.
%The first statement is true simply because at the linearization point of \acquire{} (Line \ref{line:lockfree_acquire_get}), we read the current index and version number, which came from the last \set{}. In Line \ref{line:lockfree_acquire_CAS}, if they do not match, we go back to the beginning of the loop and read the version again. Hence at this point, $i$ is the most recent version.
\end{proof}

\begin{lemma}
\label{lem:lockfree-1}
If a \release[v]() operation $R$ returns \true, then $v$ is live before the linearization point of $R$ and not live after.
%For a version with index $i$ and version number $V$, if the \release$(i)$ returns true, then version $V$ changes from live to not live.
\end{lemma}

\begin{proof}
By Observation \ref{lem:ss2}, $v$ must be live before the linearization point of $R$.

We first show that any \acquire[v] operation linearized before $R$ must have increased the counter of $v$ on Line \ref{line:lockfree_acquire_CAS1} before the linearization point of $R$. Note that after the linearization point of $R$, $S[v.index].v = empty$, meaning that the counter of $v$ can only increment before the linearization point of $R$. Therefore all \acquire[v] operations must increment the counter of $v$ before the linearization point of $R$.

Next, we show that all \acquire[v] operations linearized before $R$ have corresponding \release[v] operations that are also linearized before $R$. We know that $S[v.index] = \langle v, 0\rangle$ immediately before the linearization point of $R$, so each \acquire[v] operations linearized before $R$ has a corresponding \release[v] operation that decrements the count for $v$ before the linearization point of $R$. By Lemma \ref{lem:lf_unique}, all \release[v] operations other than $R$ return \false{} and are linearized when they decrement the count for $v$. Therefore all \acquire[v] operations linearized before $R$ have corresponding \release[v] operations that are also linearized before $R$.

We can see from the code that $v$ is not the current version at the linearization point of $R$ because $R$ passed the check in line \ref{line:lockfree_release_condition}. Combining this fact with the previous fact that we showed, we have that $v$ is not live after $R$.
\end{proof}
% We then show that for a \release{} returns true, any \release{}s on the same version must be linearized before it. Any \release{} that does not decrease counter to $0$ must happen before some \release{} that decrease the counter to $0$, so we only consider all the \release{}s that decrease the counter to $0$.
% We call them the ``almost-last'' \release{}s on the corresponding version. Only one of them will reach and succeed in \gc{}'s CAS.
% In the corresponding \gc{}, the winner passes the condition in Line \ref{line:lockfree_gc_abort}, which means that the counter has already been set to $0$ again.
% This simply indicates that all the other almost-last \release{}s must have reached the CASes in \release{} (Line \ref{line:lockfree_release_CAS}), which are their linearization points.

% Finally, once a \release{} returns \true{} on version $V$, the version will never be \acquire{}d by any further readers because the CAS in \acquire{} (Line \ref{line:lockfree_acquire_CAS}) will fail.


\begin{lemma}
\label{lem:lockfree-2}
If a \release[v]() operation $R$ returns \false, then $v$ is live after the linearization point of $R$.
\end{lemma}
\begin{proof}
Recall that $R$ is linearized at CAS on line \ref{line:lockfree_release_CAS} that decrements the count of $v$. By Observation \ref{lem:ss2}, we know that $v$ is live just before this CAS. Therefore to show that $v$ is live immediately after this CAS, it suffices to show that $v$ is live at some configuration after this CAS (By Observation \ref{lem:ss1}).

If $R$ returns on line \ref{line:lockfree_release_condition}, then either $v = \currentv$, in which case $v$ is live by definition, or the count of $v$ is non-zero immediately after the linearization point of $R$, in which case $v$ is live by Lemma \ref{lem:lf_live}.

If $R$ returns on line \ref{line:lockfree_gc_abort} or line \ref{line:lockfree_gc_CAS}, then either some \release[v]() operation $R'$ is linearized before the end of $R$ or the count of $v$ is non-zero at some point after the linearization point of $R$. In the later case, we know that $v$ is live after the linearization point of $R$ by Lemma \ref{lem:lf_live}. In the former case, we know that $R'$ must be linearized after $R$ because $v$ is live before the linearization point of $R$ and $v$ is not live after the linearization point of $R'$ (by Lemma \ref{lem:lockfree-1}). By Observation \ref{lem:ss2}, $v$ is live immediately before the linearization point of $R'$, so $v$ must have been live after the linearization point of $R$.
%We show when \release{} returns false, the version stays live for a while after its linearization point, which is the CAS in Line \ref{line:lockfree_release_CAS}. We look at the corresponding successful \release{} on the same version. If the successful one comes later, at this point its corresponding \acquire{} has not been \release{}d yet, and by definition the version is live.
%Otherwise, the successful one comes before it, that is not possible because by Lemma \ref{lem:lockfree-1} the version became not live then.
%If it is returned by Line \ref{line:lockfree_release_false}, this means that there are other processors working on it (i.e., there is some \acquire{} that has not been \release{}d yet). In this case it stays live by definition. Otherwise, the \false{} is returned by \gc{}, which means that this \release{} is almost-last. In this case, the \release{} returning \true{} can not finish before the CAS of the current \release{} because otherwise the counter will be more than $0$.
\end{proof}

Together, Lemmas \ref{lem:lockfree-acquire}, \ref{lem:lockfree-1} and \ref{lem:lockfree-2}, and Definition \ref{def:lf_linpoint} directly imply Theorem \ref{thm:lockfree-lin}.
\end{maybeappendix}





==> old/model.tex <==
\subsection{Set-Up}

%The machine model we consider is an asynchronous shared memory with $P$ processors.
%%PRAM.  In the model we have $P$ processors sharing a sequentially consistent memory.
%The memory instructions supported are atomic read, write and CAS to arbitrary locations.
%%Each processor can proceed at its own pace and any processor can be delayed arbitrarily.  
%We use \emph{work} to refer to a count of instructions
%that are executed.  This could either be on a single processor or summed
%across processors -- i.e. if 10 processors each run 10 instructions,
%the work is 100.  The \emph{machine work} is with respect to machine
%instructions. 
%Where specified, we also consider \emph{contention work}, which is the total amount of contention experienced by all \op{}s.
%as in the definition of work in \cite{ben2017analyzing} or stalls in \cite{fich2005linear}.

\Naama{Formalize the following, in terms of a linearizable version maintenance object.}

A \emph{transaction} is a piece of code that accesses a database via read and/or write instructions to shared objects. 
Each transaction begins with an invocation and ends with a response. It is \emph{live} from the invocation until the response.
In our model, each transaction is composed of the following phases: \emph{acquire}, \emph{body}, \emph{release}, and a possible \emph{GC} phase at the end. The body of the transaction is specified by the user, and is called the \emph{user code}. The rest of the phases are designed to efficiently maintain and collect multiple versions to allow for quick access to the data.
We require that user code in transactions only access shared memory via pure pointer machine instructions.  
Each transaction is also allowed to access local memory, in which we allow the user code to use either pointer-machine instructions or standard RAM instructions.
One of the goals of the paper is to show that we can simulate the instructions efficiently on a RAM even with multiple versions. 
The \emph{user work} is the number of pointer machine instructions and other local instructions done in the body of transactions.

A \emph{version} is a pointer to a tuple, such
that the data reachable using LISP machine instructions from the version constitutes the whole state of the
shared world that is visible to a transaction. Every transaction $t$ uses exactly one version $V(t)$.
Each transaction must call an \acquire[] \op{} to acquire a version to work on, and \release[] when it is done, to release the version. 
A transaction that has only read instructions on the database (that is, other than its \acquire[], \release[]) is called a \emph{read transaction}. Otherwise, it is called a \emph{write transaction}.
Write transactions must also call a \set[] \op{} before calling \release[], in order to commit a new version and make it visible to new transactions. 
We only allow a single write transaction at a time. That is, the intervals of write transactions may not overlap with one another.  
The \acquire[], \release[], and \set[] \op{}s are not part of the user code and are described in detail in this paper.

The \emph{acquire}
phase of a transaction goes from the invocation until the return of the call to
\texttt{acquire}; the \emph{body} runs the user code;
the \emph{release} phase goes from the call to \texttt{release} until a
point at which a committed version is visible to other
transactions; and finally the \emph{GC} phase that possibly collects some garbage and finishes at the response.   We assume the transactions can have other channels to the outside world so
they can output their result.   This can precede the release phase.
Thus any results of a read transaction are available at the end of the body.


%\Naama{Note that this is NOT the standard way of defining a transaction (with acquire, release, GC, etc.) Should this be moved to the model section? If so, how much should we say about transactions in the prelims?}

Each transaction is associated with a processor $p_1, \ldots, p_P$ and
only one transaction can be live on a processor at a given time.  
A \emph{transactional
	history} is an interleaved sequence of steps (invocations, acquired
points (at end of acquire phase), release points (at start of
release phase), commit points (at end of release phase), and responses) for a
set of transactions.  
A \emph{sequential transactional history} is a history in which the steps of one transaction are never interleaved with the steps of another.
Note that the definition of a transactional history is similar to an object history, except that transactions execute several instructions on several objects, instead of just one instruction and object.
%A \emph{transactional history} and a \emph{sequential transactional history} are defined similarly to object histories, with the difference that transactions execute several instructions on several objects, instead of just one instruction and object.
%A transactional history is said to be \emph{equivalent} to a sequential transactional history if, after removing all aborted transactions, the sequence of transactions in the two histories is the same.
A transactional history $H$ is \emph{serializable} if there is some sequential transactional history $S$ that is equivalent to it. It is \emph{strictly serializable} if $<_S$ is an extension of $<_h$. 

Two instructions are concurrent in a history if they are in different transactions
and are not separated by the response of the transaction of one, and
then the invocation of the transaction of the other.    Access to a memory
location is \emph{contention free} in a history if no concurrent
instruction does a write to the memory location.    An instruction in
a program is contention free if for all possible histories it is
contention free. 
%
%A \emph{version} is a pointer to a tuple, such
%that the data reachable from the version constitutes the whole state of the
%shared world that is visible to a transaction.  A transaction runs
%\texttt{acquire} at its start which gives it a version to work on.  A
%read-only transaction runs \texttt{release} at its end to release
%access to its version.  A read-write transaction runs a
%\texttt{commit}$(v)$ at its end which releases the old version and commits a new
%version $v$.   Every transaction $t$ uses exactly one version $V(t)$.




==> old/overall.tex <==
\section{Garbage Collection}\label{sec:gc}

%\subsection{Garbage Collection}

%We now discuss how garbage collection is done in our transactional database.
In our transactional database, each transaction of the user is wrapped with calls to a version maintenance object to acquire a version for access, and to release it at the end. A write transaction also calls \set[] in order to commit the new version. If a transaction's \release[v] operation returns \true, then it also calls \collect{} to garbage collect its version before terminating.

We now present the \collect{} operation, and prove that this scheme guarantees safe and precise garbage collection. Furthermore, we show that our garbage collection mechanism is efficient; %even when accounting for contention \Naama{can we actually show this?}, 
garbage collecting takes $O(v)$ machine work, where $v$ is the size of the version being collected.  

The writer uses path copying to create a new version. This means that while each version has a unique root, many versions might share subsets of the database (the paths that did not change from version to version). In order to allow collecting a single version later on, reference counts need to be kept on the nodes of the database.
The counts are incremented only by the writer.
When copying a path, it increments the counters of all nodes that the new path points to. That is, each node's count indicates how many nodes in the database point to it, including copies in different versions.
%It must increment the counts of all nodes that are not on a path that it copied, and set the counts of each copied node to $1$ \Naama{note that this means that the writer actually does have to access the entire database.}. 
In this way, processes executing a \collect{} first decrement the count of each node in their version, and only actually collect the ones whose count has reached zero. 

The simplest way of implementing the counters is via a fetch-and-add object per node. This is what we use in this paper. However, we note that this could introduce unnecessary contention. To mitigate that effect, other options, like dynamic non-zero indicators \cite{acar2017contention}, can be used. 
% this could introduce a lot of contention; if $k$ versions are being simultaneously collected and they all share some nodes, then they could all contend, experiencing up to $k$ contention each on every node that they share.

%To reduce the contention, reference counting can be done with a dynamic scalable non-zero indicator (SNZI) object \cite{acar2017contention} instead. This object allows lock-free increments and decrements. Rather than keeping an exact count, a non-zero indicator has a \emph{query} instruction, which is wait-free, and returns a boolean value indicating whether or not its current count is exactly $0$ \cite{ellen2007snzi}. This interface is all we need for the purpose of reference counting, since a process only needs to take action when the count reaches zero. This weakening of the counter specification allows the dynamic SNZI object to mitigate contention.
%In fact, the dynamic SNZI object can guarantee constant amortized contention and work per access. However, this strong guarantee comes at a cost; the SNZI object itself could require a lot of space. In particular, to guarantee constant contention, the dynamic SNZI object must have size proportional its total count at any point in time, that is, the number of copies of it in the database.
%However, Acar \textit{et al.} also show how to trade off contention for space using the dynamic SNZI object \cite{acar2017contention}. If we allow for up to $O(t)$ amortized contention per access, dynamic SNZI can be built using space at most $O(count/t)$.

\begin{theorem}
	Our garbage collecting mechanism is safe and precise, and takes $O(v)$ machine instructions to collect a version of size $v$.
\end{theorem}
%
%\begin{theorem}
%	We guarantee $O(v)$ machine work, and up to $O(\ldots)$ contention work.
%\end{theorem}
%
%\begin{theorem}
%	When using dynamic SNZI, we guarantee $O(v)$ machine work, and up to $O(\ldots)$ contention work, in $O(\ldots)$ space.
%\end{theorem}

%In particular, there must be communication between the incrementing processor and the decrementing processor on the same location. The dynamic SNZI it allows for a trade-off between contention and space.

==> other-vm-algs.tex <==

\renewcommand{\figurename}{Algorithm}
%\lstset{basicstyle=\footnotesize\ttfamily, tabsize=2, escapeinside={@}{@}}
\lstset{literate={<}{{$\langle$}}1  {>}{{$\rangle$}}1}

\begin{figure*}[!t!h]
	\caption{RCU algorithm for the Version Maintenance Problem}

\begin{minipage}{0.48\textwidth}
\begin{lstlisting}[countblanklines=false]
struct Version{
	int timestamp;
	int index; 
	};
struct Announcement {
	Version v; 
	};

Version V;
Announcement A[P];
Data* D[3P+1];
Version empty = <-1, -1>;

Data* getData(Version v) {
	return D[v.index];}

Data* acquire(int k) {
	rcu_read_lock();
	A[k].v = V;
	return getData(A[k].v);
}	
\end{lstlisting}
\end{minipage}\hfill
\begin{minipage}{0.49\textwidth}
\begin{lstlisting}[countblanklines=false,firstnumber=33]
bool release(int k) {
	rcu_read_unlock();
	return @\bot@; }

bool set(int k, Data* data) {
	Version oldVer = A[k].v; //the version you acquired
	Version newVer;
	for(int i = 0; i @$<$@ 3P+1; i++) {
		if(S[i] == <empty, 0>) {
			newVer = <V.timestamp+1, i>;
			if(CAS(S[i], <empty, 0>, <newVer,0>)) {
				D[i]=data;
				break;	}   }	
		if(i == 3P) return false; }

	if(CAS(V, oldVer, newVer)) {
		rcu_synchronize();
		return {oldVer};
	}
	else
		return false;
}
\end{lstlisting}
\end{minipage}
\label{alg:waitfree}
\end{figure*}

\renewcommand{\figurename}{Figure}




\renewcommand{\figurename}{Algorithm}
%\lstset{basicstyle=\footnotesize\ttfamily, tabsize=2, escapeinside={@}{@}}
\lstset{literate={<}{{$\langle$}}1  {>}{{$\rangle$}}1}

\begin{figure*}[!t!h]
	\caption{Epoch algorithm for the Version Maintenance Problem}

\begin{minipage}{0.48\textwidth}
\begin{lstlisting}[countblanklines=false]
Data* V;
int A[P];
int Epoch;
List RetiredList[P][3];

List combine_lists(int idx) {
	List list = EMPTY_LIST;
	for(int i = 0; i < P; i++)
		list = combine(list, Retiredlist[i][idx]);
}

Data* acquire(int k) {
	A[k] = Epoch;
	return V;
}	
\end{lstlisting}
\end{minipage}\hfill
\begin{minipage}{0.49\textwidth}
\begin{lstlisting}[countblanklines=false,firstnumber=33]
List release(int k) {
	int cur_epoch = A[k];
	for(int i = 0; i < P; i++)
		if(A[i] != cur_epoch) return EMPTY_LIST;
	if(epoch == cur_epoch && CAS(epoch, cur_epoch, cur_epoch+1))
	{
		int idx = (cur_epoch-1) % 3;
		List list = combine_lists(idx);
		for(int i = 0; i < P; i++) RetiredList[i][idx].clear();
		return list;
	}
	return EMPTY_LIST; @\label{h_one}@ }

bool set(int k, Data* data) {
	Data* old_data = V;
	if(CAS(V, old_data, data)) {
		int idx = A[k] % 3;
		RetiredList[k][idx].add(old_data);
		return true;
	}
	else
		return false;
}
\end{lstlisting}
\end{minipage}
\label{alg:waitfree}
\end{figure*}

\renewcommand{\figurename}{Figure}





\renewcommand{\figurename}{Algorithm}
%\lstset{basicstyle=\footnotesize\ttfamily, tabsize=2, escapeinside={@}{@}}
\lstset{literate={<}{{$\langle$}}1  {>}{{$\rangle$}}1}

\begin{figure*}[!t!h]
	\caption{Hazard pointer based algorithm for the Version Maintenance Problem}

\begin{minipage}{0.48\textwidth}
\begin{lstlisting}[countblanklines=false]
Data* V;
Data* A[P];
List retired_list[P];
List safe_to_free[P];

void scan(int k) {
	HashTable h;
	for(int i = 0; i < P; i++) h.add(A[i]);
	List list;
	for(each node in retired_list[k]) {
		if(h.contains(node->data))
			list.add(node->data);
		else
			safe_to_free[k].add(node->data); }
	retired_list[k] = list;
}

void retire(int k, Data* data) {
	retired_list[k].add(data);
	if(retire_list[k].size() == 2P)
		scan(k);
}

Data* acquire(int k) {
	while (A[k] != V) A[k] = V;
	return A[k];
}	
\end{lstlisting}
\end{minipage}\hfill
\begin{minipage}{0.49\textwidth}
\begin{lstlisting}[countblanklines=false,firstnumber=33]
List release(int k) {
	A[k] = NULL;
	List ret = safe_to_free[k];
	safe_to_free[k].clear();
	return ret; }

bool set(int k, Data* data) {
	Data* old_data = V;
	if(CAS(V, old_data, data)) {
		retire(k, old_data);
		return true;
	}
	else
		return false;
}
\end{lstlisting}
\end{minipage}
\label{alg:waitfree}
\end{figure*}

\renewcommand{\figurename}{Figure}

==> version_test.tex <==
\section{The Version Maintenance Problem}

We abstract what we need to maintain multiple versions as the
\emph{version maintenance} problem.      The problem is to support a
data structure with three operations: \set, \acquire[v] and \release.
The \set$(a)$ creates a new version with value $a$ and sets it as the
current version.     The \acquire$(k)$ acquires the current version for
process $k, 1 \leq k \leq P$ and returns its value.   The \release$(k)$ releases the acquired
version for process $k$.    For a given $k$ the \acquire$(k)$ and
\release$(k)$ must alternate starting with an \acquire{}. 
We say that a process $k$ has \emph{acquired} version $v$ if \acquire$(k)$ returns $v$, and we say $k$ has \emph{released} $v$ when the next \release$(k)$ operation returns.
